Copilot-in-the-Loop: Fixing Code Smells in Copilot-Generated Python Code using Copilot

As one of the most popular dynamic languages, Python experiences a decrease in readability and maintainability when code smells are present. Recent advancements in Large Language Models have sparked growing interest in AI-enabled tools for both code generation and refactoring. GitHub Copilot is one such tool that has gained widespread usage. Copilot Chat, released in September 2023, functions as an interactive tool aimed at facilitating natural language-powered coding. However, limited attention has been given to understanding code smells in Copilot-generated Python code and Copilot Chat's ability to fix the code smells. To this end, we built a dataset comprising 102 code smells in Copilot-generated Python code. Our aim is to first explore the occurrence of code smells in Copilot-generated Python code and then evaluate the effectiveness of Copilot Chat in fixing these code smells employing different prompts. The results show that 8 out of 10 types of code smells can be detected in Copilot-generated Python code, among which Multiply-Nested Container is the most common one. For these code smells, Copilot Chat achieves a highest fixing rate of 87.1%, showing promise in fixing Python code smells generated by Copilot itself. In addition, the effectiveness of Copilot Chat in fixing these smells can be improved by providing more detailed prompts.

==> table_overall_fixing_rate.tex <==
\begin{table}[hbp]
\scriptsize
\caption{Counts of fixed and unfixed code smells using different prompts.}
\label{The numbers of fixed and unfixed code smells using different prompts}
\begin{tabular}{m{3.9cm}m{0.7cm}<{\centering}m{1cm}<{\centering}m{1.7cm}<{\centering}}
\toprule
\textbf{Prompt}                 & \textbf{\#Fixed}   & \textbf{\#Unfixed} & \textbf{Fixing Rate} \\ \hline
General Fix Prompt              & 32                 & 61                 & 34.4\%               \\ \hline
Code Smell Fix Prompt           & 60                 & 33                 & 64.5\%               \\ \hline
Specific Code Smell Fix Prompt  & 81                 & 12                 & 87.1\%               \\ \bottomrule
\end{tabular}
\end{table}
